FLEA: Provably Robust Fair Multisource Learning from Unreliable Training Data

Fairness-aware learning aims at constructing classifiers that not only make accurate predictions, but also do not discriminate against specific groups. It is a fast-growing area of machine learning with far-reaching societal impact. However, existing fair learning methods are vulnerable to accidental or malicious artifacts in the training data, which can cause them to unknowingly produce unfair classifiers. In this work we address the problem of fair learning from unreliable training data in the robust multisource setting, where the available training data comes from multiple sources, a fraction of which might not be representative of the true data distribution. We introduce FLEA, a filtering-based algorithm that identifies and suppresses those data sources that would have a negative impact on fairness or accuracy if they were used for training. As such, FLEA is not a replacement of prior fairness-aware learning methods but rather an augmentation that makes any of them robust against unreliable training data. We show the effectiveness of our approach by a diverse range of experiments on multiple datasets. Additionally, we prove formally that -- given enough data -- FLEA protects the learner against corruptions as long as the fraction of affected data sources is less than half. Our source code and documentation are available at https://github.com/ISTAustria-CVML/FLEA.

==> TMLR-corrected-arxiv_arXiv_test <==
@string{JOE = "Journal of Econometrics"}
@string{TPA = "Theory of Probability \& Its Applications"}
@string{AOS = "Annals of Statistics"}
@string{TVP = "Teoriya Veroyatnostei i ee Primeneniya"}
@string{AAP = "Advances in Applied Probability"}
@string{TNSE = "IEEE Transactions on Network Science and Engineering (TNSE)"}
@string{TKDE = "IEEE Transactions on Knowledge and Data Engineering (TKDE)"}

@string{TOIS = "ACM Transactions on Information Systems (TOIS)"}
@string{DMKD = "Data Mining and Knowledge Discovery (DMKD)"}
@string{SICOMP = "SIAM Journal on Computing (SICOMP)"}
@string{JACM = "Journal of the ACM (JACM)"}
@string{TCC = "Theoretical Computer Science (TCC)"}
@string{JMLR = "Journal of Machine Learning Research (JMLR)"}
@string{TMLR = "Transactions of Machine Learning Research (TMLR)"}
@string{KAIS = "Knowledge and Information Systems (KAIS)"}}

@string{CVPR = "Conference on Computer Vision and Pattern Recognition (CVPR)"}
@string{ECCV = "European Conference on Computer Vision (ECCV)"}
@string{ICCV = "International Conference on Computer Vision (ICCV)"}
@string{NIPS = "Conference on Neural Information Processing Systems (NeurIPS)"}
@string{NeurIPS = "Conference on Neural Information Processing Systems (NeurIPS)"}
@string{ICML = "International Conference on Machine Learing (ICML)"}
@string{COLT = "Workshop on Computational Learning Theory (COLT)"}
@string{UAI = "Uncertainty in Artificial Intelligence (UAI)"}
@string{ECML = "European Conference on Marchine Learning (ECML)"}
@string{ECMLPKDD = "European Conference on Machine Learning and Data Mining (ECML PKDD)"}
@string{AISTATS = "Conference on Uncertainty in Artificial Intelligence (AISTATS)"}
@string{ALT = "Algorithmic Learning Theory (ALT)"}
@string{AAAI = "Conference on Artificial Intelligence (AAAI)"}
@string{IJCAI = "International Joint Conference on Artificial Intelligence (IJCAI)"}
@string{SODA = "Symposium on Discrete Algorithms (SODA)"}
@string{ICLR = "International Conference on Learning Representations (ICLR)"}
@string{EMNLP = "Conference on Empirical Methods on Natural Language Processing (EMNLP)"}
@string{SIGIR = "International Conference on Research and Development in Information Retrieval (SIGIR)"}
@string{SIGMOD = "International Conference on Management of Data (SIGMOD)"}
@string{WSDM = "International Conference on Web Search and Data Mining (WSDM)"}
@string{ITCS = "Innovations in Theoretical Computer Science Conference (ITCS)"}
@string{RECSYS = "Conference on Recommender Systems (RecSys)"}
@string{FACCT = "Conference on Fairness, Accountability and Transparency (FAccT)"}
@string{FAT = "Conference on Fairness, Accountability and Transparency (FAccT)"}
@string{FATML = "Fairness, Accountability, and Transparency in Machine Learning (FAT/ML)"}
@string{SSDMC = "Scientific and Statistical Database Management Conference (SSDBM)"}
@string{WWW = "International World Wide Web Conference (WWW)"}
@string{COMAD = "International Conference on Management of Data (COMAD)"}
@string{CHI = "Conference on Human Factors in Computing Systems (CHI)"}
@string{CIKM = "Conference on Information and Knowledge Management (CIKM)"}
@string{AIES = "Conference on AI, Ethics, and Society (AIES)"}
@string{STOC = "Symposium on Theory of Computing (STOC)"}

@string{CP = "International Conference on Principles and Practice of Constraint Programming (CP)"}

@string{ACL = "Annual Meeting of the Association for Computational Linguistics (ACL)"}
@string{KDD = "Conference on Knowledge Discovery and Data Mining (KDD)"}
@string{PKDD = "European Conference on Principles and Practice of Knowledge Discovery in Databases (PKDD)"}
@string{VLDB = "International Conference on Very Large Data Bases (VLDB)"}
@string{IJCV = "International Journal of Computer Vision (IJCV)"}
@string{ML = "Machine Learning (ML)"}

@string{WILEY = "Wiley"},
@string{WILEYSONS = "John Wiley \& Sons"}
@string{MIT = "The MIT Press"},
@string{CAMBRIDGE = "Cambridge University Press"},
@string{SPRINGER = "Springer"},
@string{KLUWER = "Kluwer Academic Press"}
@string{ELSEVIER = "Elsevier"}
@string{OXFORD = "Oxford University Press"},

@book{halmos2013measure,
  title={Measure Theory},
  author={Halmos, Paul R.},
  novolume={18},
  year={2013},
  publisher=SPRINGER
}

@article{friedman2001greedy,
  title={Greedy function approximation: a gradient boosting machine},
  author={Friedman, Jerome H},
  journal=AOS,
  nopages={1189--1232},
  year={2001},
}
@article{student1908probable,
  title={The probable error of a mean},
  author={Student},
  journal={Biometrika},
  nopages={1--25},
  year={1908},
  publisher={JSTOR}
}
@article{JMLR:v13:gretton12a,
  author  = {Arthur Gretton and Karsten M. Borgwardt and Malte J. Rasch and Bernhard Sch{{\"o}}lkopf and Alexander Smola},
  title   = {A Kernel Two-Sample Test},
  journal = JMLR,
  year    = {2012},
  novolume  = {13},
  nonumber  = {25},
  nopages   = {723-773},
  nourl     = {http://jmlr.org/papers/v13/gretton12a.html}
}
@book{villani2009optimal,
  title={Optimal transport: old and new},
  author={Villani, C{\'e}dric},
  novolume={338},
  year={2009},
  publisher=SPRINGER
}
@book{Tsybakov:1315296,
      author        = "Tsybakov, Alexandre B",
      title         = "{Introduction to Nonparametric Estimation}",
      publisher     = SPRINGER,
      noaddress       = "Dordrecht",
      series        = "Springer series in statistics",
      year          = "2009",
}
@article{kullback1951information,
  title={On information and sufficiency},
  author={Kullback, Solomon and Leibler, Richard A},
  journal={The Annals of Mathematical Statistics},
  novolume={22},
  nonumber={1},
  nopages={79--86},
  year={1951},
  nopublisher={JSTOR}
}

@book{corder2014nonparametric,
  title={Nonparametric statistics: A step-by-step approach},
  author={Corder, Gregory W and Foreman, Dale I},
  year={2014},
  publisher=WILEYSONS
}

@inproceedings{ding2021retiring,
  title={Retiring Adult: New Datasets For Fair Machine Learning},
  author={Ding, Frances and Hardt, Moritz and Miller, John and Schmidt, Ludwig},
  booktitle=NeurIPS,
  year={2021}
}

@inproceedings{konstantinov2020sample,
  title={On the sample complexity of adversarial multi-source {PAC} learning},
  author={Konstantinov, Nikola and Frantar, Elias and Alistarh, Dan and Lampert, Christoph},
  booktitle=ICML,
  year={2020}
}




@inproceedings{erfani2017shared,
  title={From shared subspaces to shared landmarks: A robust multi-source classification approach},
  author={Erfani, Sarah and Baktashmotlagh, Mahsa and Moshtaghi, Masud and Nguyen, Vinh and Leckie, Christopher and Bailey, James and Ramamohanarao, Kotagiri},
  booktitle=AAAI,
  novolume={31},
  nonumber={1},
  year={2017}
}

@inproceedings{li2021tilted,
  title={Tilted empirical risk minimization},
  author={Tian Li and Ahmad Beirami and Maziar Sanjabi and Virginia Smith},
  booktitle=ICLR,
  year={2021}
}

% Related works - fairness

@inproceedings{calders2009parity,
  title={Building classifiers with independency constraints},
  author={Calders, Toon and Kamiran, Faisal and Pechenizkiy, Mykola},
  booktitle={International Conference on Data Mining Workshops (IDCMW)},
  year={2009}
}

@inproceedings{mehrabi2020exacerbating,
  title={Exacerbating Algorithmic Bias through Fairness Attacks},
  author={Mehrabi, Ninareh and Naveed, Muhammad and Morstatter, Fred and Galstyan, Aram},
  booktitle=AAAI,
  year={2021}
}

@inproceedings{kallus2019assessing,
  title={Assessing algorithmic fairness with unobserved protected class using data combination},
  author={Kallus, Nathan and Mao, Xiaojie and Zhou, Angela},
  booktitle=FACCT,
  year={2020}
}

@inproceedings{agarwal2018reductions,
  title={A Reductions Approach to Fair Classification},
  author={Agarwal, Alekh and Beygelzimer, Alina and Dudik, Miroslav and Langford, John and Wallach, Hanna},
  booktitle=ICML,
  year={2018}
}

@inproceedings{celis2021fair,
  title={Fair Classification with Noisy Protected Attributes: A Framework with Provable Guarantees},
  author={L. Elisa Celis and Lingxiao Huang and Vijay Keswani and Nisheeth K. Vishnoi},
  booktitle=ICML,
  year={2021}
}

@inproceedings{kamishima2011fairness,
  title={Fairness-aware learning through regularization approach},
  author={Kamishima, Toshihiro and Akaho, Shotaro and Sakuma, Jun},
  booktitle={International Conference on Data Mining Workshops (IDCMW)},
  year={2011}
}
@inproceedings{kamishima2012fairness,
  title={Fairness-aware classifier with prejudice remover regularizer},
  author={Kamishima, Toshihiro and Akaho, Shotaro and Asoh, Hideki and Sakuma, Jun},
  booktitle=ECMLPKDD,
  nopages={35--50},
  year={2012},
  noorganization={Springer}
}


@inproceedings{lamy2019noise,
  title={Noise-tolerant fair classification},
  author={Lamy, Alex and Zhong, Ziyuan and Menon, Aditya K and Verma, Nakul},
  booktitle=NeurIPS,
  nopages={294--306},
  year={2019}
}

% Related works - fairness - postprocessing methods

@inproceedings{Hardt2016Equality,
  title={Equality of Opportunity in Supervised Learning},
  author={Moritz Hardt and Eric Price and Nathan Srebro},
  booktitle=NeurIPS,
  year={2016}
}

@inproceedings{Chzhen2020FairRegressionWasserstein,
 title={Fair regression with {Wasserstein} barycenters},
 author={Chzhen, Evgenii and Denis, Christophe and Hebiri, Mohamed and Oneto, Luca and Pontil, Massimiliano},
 booktitle=NeurIPS,
 year={2020}
}

% Related works - fairness - penalty methods

@InProceedings{zafar17FairnessConstraints,
  title={Fairness Constraints: Mechanisms for Fair Classification},
  author={Muhammad Bilal Zafar and Isabel Valera and Manuel Gomez Rogriguez and Krishna P. Gummadi},
  booktitle=AISTATS,
  year={2017}
}

@inproceedings{Mandal2020EnsuringFairness,
 title={Ensuring Fairness Beyond the Training Data},
 author={Mandal, Debmalya and Deng, Samuel and Jana, Suman and Wing, Jeannette and Hsu, Daniel J},
 booktitle=NeurIPS,
 year = {2020}
}

@inproceedings{chuang2021fair,
  title={Fair Mixup: Fairness via Interpolation},
  author={Ching-Yao Chuang and Youssef Mroueh},
  booktitle=ICLR,
  year={2021},
}

% Related works - fairness - Adversarial Methods

@inproceedings{zhang2018MitigatingBiasAdversarial,
  title={Mitigating Unwanted Biases with Adversarial Learning},
  author={Zhang, Brian Hu and Lemoine, Blake and Mitchell, Margaret},
  booktitle=AIES,
  year={2018}
}

@inproceedings{Lahoti2020AdversarialReweighting,
  title={Fairness without Demographics through Adversarially Reweighted Learning},
  author={Lahoti, Preethi and Beutel, Alex and Chen, Jilin and Lee, Kang and Prost, Flavien and Thain, Nithum and Wang, Xuezhi and Chi, Ed},
  booktitle=NeurIPS,
  year={2020}
}


@inproceedings{beutel2017data,
  title={Data Decisions and Theoretical Implications when Adversarially Learning Fair Representations},
  author={Alex Beutel and Jilin Chen and Zhe Zhao and Ed H. Chi},
  booktitle=FACCT,
  year={2017}
}

@inproceedings{wadsworth2018,
  title={Achieving Fairness through Adversarial Learning: an Application to Recidivism Prediction}, 
  author={Christina Wadsworth and Francesca Vera and Chris Piech},
  booktitle=FACCT,
  year={2018}
}

% Related works - fairness -  filtering Methods
@InProceedings{roh20FRtrain,
  title={{FR}-Train: A Mutual Information-Based Approach to Fair and Robust Training},
  author={Roh, Yuji and Lee, Kangwook and Whang, Steven and Suh, Changho},
  booktitle=ICML,
  year={2020}
}

% Related works - fairness -  filtering Methods
@InProceedings{roh2021sample,
  title={Sample Selection for Fair and Robust Training},
  author={Roh, Yuji and Lee, Kangwook and Whang, Steven and Suh, Changho},
  booktitle=NeurIPS,
  year={2021}
}

@InProceedings{blum2020recovering,
  title={Recovering from biased data: Can fairness constraints improve accuracy?},
  author={Avrim Blum and Kevin Stangl},
  booktitle={Symposium on the Foundations of Responsible Computing (FORC)},
  year={2020}
}

% Fair+robust classification:  label changes
@InProceedings{blum2020recovering,
  title={Recovering from biased data: Can fairness constraints improve accuracy?},
  author={Avrim Blum and Kevin Stangl},
  booktitle={Symposium on the Foundations of Responsible Computing (FORC)},
  year={2020}
}
@InProceedings{biswas2021ensuring,
  title = {Ensuring Fairness under Prior Probability Shifts},
  author = {Arpita Biswas and Suvam Mukherjee},
  booktitle = {Conference on Artificial Intelligence, Ethics, and Society (AIES)},
  year = {2021}
}

% Fair classification: others

@inproceedings{cho2020fair,
  title={A fair classifier using kernel density estimation},
  author={Cho, Jaewoong and Hwang, Gyeongjo and Suh, Changho},
  booktitle=NeurIPS,
  year={2020}
}


@inproceedings{tan2020learning,
  title={Learning fair representations for kernel models},
  author={Tan, Zilong and Yeom, Samuel and Fredrikson, Matt and Talwalkar, Ameet},
  booktitle=AISTATS,
  year={2020}
}





% Related works - General learning from multisourceish or different distributions data
@inproceedings{pmlr-v97-mahloujifar19a,
  title={Universal Multi-Party Poisoning Attacks},
  author={Mahloujifar, Saeed and Mahmoody, Mohammad and Mohammed, Ameer},
  booktitle=ICML,
  year={2019},
}

@inproceedings{qiao2018outliers,
  title={Do Outliers Ruin Collaboration?},
  author={Qiao, Mingda},
  booktitle=ICML,
  year={2018}
}

@inproceedings{mehrotra2021setselection,
  title={Mitigating Bias in Set Selection with Noisy Protected Attributes},
  author={Mehrotra, Anay and Celis, L. Elisa},
  booktitle=FACCT,
  year={2021},
}

@inproceedings{wang2020robustfairnessnoise,
  title={Robust Optimization for Fairness with Noisy Protected Groups},
  author={Wang, Serena and Guo, Wenshuo and Narasimhan, Harikrishna and Cotter, Andrew and Gupta, Maya and Jordan, Michael},
  booktitle=NeurIPS,
  year={2020}
}

@article{cortes_adaptation,
  title={Adaptation Based on Generalized Discrepancy},
  author={Corinna Cortes and Mehryar Mohri and Andr{{\'e}}s Mu{{\~n}}oz Medina},
  journal=JMLR,
  year={2019},
}

@InProceedings{jain2020_optimalrobustlearning,
  title={Optimal Robust Learning of Discrete Distributions from Batches},
  author={Jain, Ayush and Orlitsky, Alon},
  booktitle=ICML,
  year={2020},
}

@inproceedings{chen2019efficiently,
  title={Efficiently Learning Structured Distributions from Untrusted Batches},
  author={Chen, Sitan and Li, Jerry and Moitra, Ankur},
  booktitle=STOC,
  year={2019}
}

@inproceedings{qiao2018learning,
  title={Learning Discrete Distributions from Untrusted Batches},
  author={Qiao, Mingda and Valiant, Gregory},
  booktitle=ITCS,
  year={2018},
}

@incollection{alistarh2018byzantineSGD,
  title={Byzantine Stochastic Gradient Descent},
  author={Alistarh, Dan and Allen-Zhu, Zeyuan and Li, Jerry},
  booktitle=NeurIPS,
  year={2018},
}

@inproceedings{allenzhu2021byzantine,
  title={Byzantine-Resilient Non-Convex Stochastic Gradient Descent},
  author={Zeyuan Allen-Zhu and Faeze Ebrahimian and Jerry Li and Dan Alistarh},
  booktitle=ICLR,
  year={2021}
}

@incollection{zhang2012generalizationNIPS,
  title={Generalization Bounds for Domain Adaptation},
  author={Zhang, Chao and Zhang, Lei and Ye, Jieping},
  booktitle=NeurIPS,
  year={2012},
}

@InProceedings{konstantinov2019robust,
  title={Robust Learning from Untrusted Sources},
  author={Konstantinov, Nikola and Lampert, Christoph H.},
  booktitle=ICML,
  year={2019},
}

@inproceedings{ushabat2020sample,
  title={Sample Complexity of Uniform Convergence for Multicalibration}, 
  author={Eliran Shabat and Lee Cohen and Yishay Mansour},
  year={2020},
  booktitle=NeurIPS,
}

@InProceedings{woodworth17learning,
  title = {Learning Non-Discriminatory Predictors},
  author = {Woodworth, Blake and Gunasekar, Suriya and Ohannessian, Mesrob I. and Srebro, Nathan},
  booktitle = COLT,
  year = {2017}
}

@inproceedings{goodfellow2014generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian J and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  booktitle=NeurIPS,
  year={2014}
}
@inproceedings{goodfellow2015explaining,
  title={Explaining and harnessing adversarial examples},
  author={Goodfellow, Ian J and Shlens, Jonathon and Szegedy, Christian},
  booktitle=ICLR,
  year={2015}
}

@inproceedings{kifer2004detecting,
  title={Detecting change in data streams},
  author={Kifer, Daniel and Ben-David, Shai and Gehrke, Johannes},
  booktitle=VLDB,
  year={2004}
}

@article{marcotte1992novel,
  title={Novel approaches to the discrimination problem},
  author={Marcotte, Patrice and Savard, Gilles},
  journal={Zeitschrift f{\"u}r Operations Research},
  year={1992}
}

@inproceedings{rezaei2020fairness,
  title={Fairness for robust log loss classification},
  author={Rezaei, Ashkan and Fathony, Rizal and Memarrast, Omid and Ziebart, Brian},
  booktitle=AAAI,
  year={2020}
}

@article{ben2010theory,
  title={A theory of learning from different domains},
  author={Ben-David, Shai and Blitzer, John and Crammer, Koby and Kulesza, Alex and Pereira, Fernando and Vaughan, Jennifer Wortman},
  journal=ML,
  year={2010}
}

@inproceedings{mohri2012new,
  title={New analysis and algorithm for learning with drifting distributions},
  author={Mohri, Mehryar and Medina, Andres Munoz},
  booktitle=ALT,
  year={2012}
}

@book{barocas-hardt-narayanan,
  title = {Fairness and Machine Learning},
  author = {Solon Barocas and Moritz Hardt and Arvind Narayanan},
  publisher = {fairmlbook.org},
  year = {2019}
}

@Book{bousquet2004advanced,
  author = {Bousquet, Olivier and Ulrike von Luxburg and Gunnar Raetsch},
  title = {Advanced lectures on machine learning : ML Summer Schools 2003, Canberra, Australia, February 2-14, 2003, Tübingen, Germany, August 4-16, 2003 : revised lectures},
  publisher = {Springer-Verlag},
  year = {2004},
  address = {Berlin, Germany},
  isbn = {978-3-540-28650-9}
 }
 
@Book{shwartz2014understanding,
  author = {Shalev-Shwartz, Shai and Shai Ben-David},
  title = {Understanding machine learning: from theory to algorithms},
  publisher = {Cambridge University Press},
  year = {2014}
 }

@misc{konstantinov2021fairness,
  title={Fairness Through Regularization for Learning to Rank}, 
  author={Nikola Konstantinov and Christoph H. Lampert},
  year={2021},
  eprint={2102.05996},
  archivePrefix={arXiv},
  primaryClass={cs.LG}
}

@article{konstantinov2022theotherone,
  title={Fairness-Aware Learning from Corrupted Data},
  author={Nikola Konstantinov and Christoph H. Lampert},
  journal   = JMLR,
  year={2022}
}
 
 
%not used



@misc{roh2020fairbatch,
  title={FairBatch: Batch Selection for Model Fairness}, 
  author={Yuji Roh and Kangwook Lee and Steven Euijong Whang and Changho Suh},
  year={2020},
  eprint={2012.01696},
  archivePrefix={arXiv},
  primaryClass={cs.LG}
}

@misc{bellamy2018aifairness,
  title={AI Fairness 360: An Extensible Toolkit for Detecting, Understanding, and Mitigating Unwanted Algorithmic Bias}, 
  author={Rachel K. E. Bellamy and Kuntal Dey and Michael Hind and Samuel C. Hoffman and Stephanie Houde and Kalapriya Kannan and Pranay Lohia and Jacquelyn Martino and Sameep Mehta and Aleksandra Mojsilovic and Seema Nagar and Karthikeyan Natesan Ramamurthy and John Richards and Diptikalyan Saha and Prasanna Sattigeri and Moninder Singh and Kush R. Varshney and Yunfeng Zhang},
  year={2018},
  eprint={1810.01943},
  archivePrefix={arXiv},
  primaryClass={cs.AI}
}




%Datasets

@misc{Angwin_compas,
   title="Machine bias: There's software used across the country to
predict future criminals and its biased against blacks.",
   url = {https://github.com/propublica/compas-analysis},
   publisher={ProPublica},
   author={Julia Aingwin and Jeff Larson and Surya Mattu  and Lauren Kirchner},
   year={2016},
   urldate = {2010-09-30}
}

@misc{UCI,
  author = "Dua, Dheeru and Graff, Casey",
  year = "2017",
  title = "{UCI} Machine Learning Repository",
  url = "http://archive.ics.uci.edu/ml",
  institution = "University of California, Irvine, School of Information and Computer Sciences"
}


@article{WOLF20171,
title = {Why We Should Have Seen That Coming: Comments on Microsoft’s Tay “Experiment,” and Wider Implications},
author = {Mary J. Wolf and Keith W. Miller and Frances S. Grodzinsky},
journal = {The ORBIT Journal},
novolume = {1},
nonumber = {2},
nopages = {1-12},
year = {2017},
}

@inproceedings{zafar2017fairness,
  title={Fairness beyond disparate treatment \& disparate impact: Learning classification without disparate mistreatment},
  author={Zafar, Muhammad Bilal and Valera, Isabel and Gomez Rodriguez, Manuel and Gummadi, Krishna P},
  booktitle=WWW,
  year={2017}
}

@inproceedings{dwork2012fairness,
  title={Fairness through awareness},
  author={Dwork, Cynthia and Hardt, Moritz and Pitassi, Toniann and Reingold, Omer and Zemel, Richard},
  booktitle=ITCS,
  nopages={214--226},
  year={2012}
}

@inproceedings{ting1997model,
  title={Model combination in the multiple-data-batches scenario},
  author={Ting, Kai Ming and Low, Boon Toh},
  booktitle=ECML,
  nopages={250--265},
  year={1997}
}

@article{breiman1996bagging,
  title={Bagging predictors},
  author={Breiman, Leo},
  journal=ML,
  year={1996}
}
@article{breiman2001random,
  title={Random forests},
  author={Breiman, Leo},
  journal=ML,
  novolume={45},
  nonumber={1},
  nopages={5--32},
  year={2001},
  nopublisher={Springer}
}

@article{kearns1993learning,
  title={Learning in the presence of malicious errors},
  author={Kearns, Michael and Li, Ming},
  journal={SIAM Journal on Computing},
  novolume={22},
  nonumber={4},
  nopages={807--837},
  year={1993},
  nopublisher={SIAM}
}

@inproceedings{freund1996experiments,
  title={Experiments with a new boosting algorithm},
  author={Freund, Yoav and Schapire, Robert E and others},
  booktitle=ICML,
  novolume={96},
  nopages={148--156},
  year={1996},
  noorganization={Citeseer}
}

@article{wang2018deep,
  title={Deep visual domain adaptation: A survey},
  author={Wang, Mei and Deng, Weihong},
  journal={Neurocomputing},
  year={2018}
}

@inproceedings{natarajan2013learning,
  title={Learning with noisy labels},
  author={Natarajan, Nagarajan and Dhillon, Inderjit S and Ravikumar, Pradeep and Tewari, Ambuj},
  booktitle=NIPS,
  novolume={26},
  nopages={1196--1204},
  year={2013}
}

@article{crammer2008learning,
  title={Learning from Multiple Sources},
  author={Crammer, Koby and Kearns, Michael and Wortman, Jennifer},
  journal=JMLR,
  novolume={9},
  nonumber={8},
  year={2008}
}

@article{pan2009survey,
  title={A survey on transfer learning},
  author={Pan, Sinno Jialin and Yang, Qiang},
  journal=TKDE,
  novolume={22},
  nonumber={10},
  nopages={1345--1359},
  year={2009}
}

@inproceedings{zemel2013learning,
  title={Learning fair representations},
  author={Zemel, Rich and Wu, Yu and Swersky, Kevin and Pitassi, Toni and Dwork, Cynthia},
  booktitle=ICML,
  nopages={325--333},
  year={2013}
}

@book{cormen2009introduction,
  title={Introduction to algorithms},
  author={Cormen, Thomas H and Leiserson, Charles E and Rivest, Ronald L and Stein, Clifford},
  year={2009},
  publisher=MIT
}

@inproceedings{solans2020poisoning,
  title = {Poisoning attacks on algorithmic fairness},
  author= {David Solans and Battista Biggio and Carlos Castillo},
  booktitle=ECMLPKDD,
  year={2020}
}


@article{imagenet,
Author = {Olga Russakovsky and Jia Deng and Hao Su and Jonathan Krause and Sanjeev Satheesh and Sean Ma and Zhiheng Huang and Andrej Karpathy and Aditya Khosla and Michael Bernstein and Alexander C. Berg and Li Fei-Fei},
Title = {{ImageNet Large Scale Visual Recognition Challenge}},
Year = {2015},
journal  = IJCV,
novolume={115},
nonumber={3},
nopages={211-252}
}

@book{vapnik2013nature,
  title={The nature of statistical learning theory},
  author={Vapnik, Vladimir},
  year={2013},
  series="Statistics for Engineering and Information Science",
  publisher=SPRINGER,
}

@Article{smith2018robustness,
  title =	"The robustness of majority voting compared to
		 filtering misclassified instances in supervised
		 classification tasks",
  author =	"Michael R. Smith and Tony R. Martinez",
  journal =	"Artificial Intelligence Review",
  year = 	"2018",
  nonumber =	"1",
  novolume =	"49",
  nopages =	"105--130",
}

@article{mehrabi2021survey,
  title={A survey on bias and fairness in machine learning},
  author={Mehrabi, Ninareh and Morstatter, Fred and Saxena, Nripsuta and Lerman, Kristina and Galstyan, Aram},
  journal={ACM Computing Surveys (CSUR)},
  novolume={54},
  nonumber={6},
  nopages={1--35},
  year={2021},
  nopublisher={ACM New York, NY, USA}
}

@inproceedings{feng2019learning,
  title={Learning to Confuse: Generating Training Time Adversarial Data with Auto-Encoder},
  author={Ji Feng and Qi-Zhi Cai and Zhi-Hua Zhou},
  booktitle=NeurIPS,
  year={2019}
}
@inproceedings{fowl2021adversarial,
  title={Adversarial Examples Make Strong Poisons},
  author={Fowl, Liam and Goldblum, Micah and Chiang, Ping-yeh and Geiping, Jonas and Czaja, Wojtek and Goldstein, Tom},
  booktitle=NeurIPS,
  year={2021}
}
@book{barnett1984outliers,
  title={Outliers in statistical data},
  author={Vic Barnett and Toby Lewis},
  publisher = WILEY,
  year={1984}
}



@inproceedings{li2021ditto,
  title={Ditto: Fair and robust federated learning through personalization},
  author={Li, Tian and Hu, Shengyuan and Beirami, Ahmad and Smith, Virginia},
  booktitle=ICML,
  year={2021}
}


@inproceedings{jain2020general,
  title={A General Method for Robust Learning from Batches},
  author={Jain, Ayush and Orlitsky, Alon},
  booktitle=NeurIPS,
  year={2020}
}

@inproceedings{celis2021adversarial,
  title={Fair Classification with Adversarial Perturbations},
  author={Celis, L Elisa and Mehrotra, Anay and Vishnoi, Nisheeth K},
  booktitle=NeurIPS,
  year={2021}
}

@inproceedings{charikar2017learning,
  title={Learning from untrusted data},
  author={Charikar, Moses and Steinhardt, Jacob and Valiant, Gregory},
  booktitle=STOC,
  year={2017}
}
@article{kamiran2012data,
  title={Data preprocessing techniques for classification without discrimination},
  author={Faisal Kamiran and Toon Calders},
  journal=KAIS,
  novolume={33},
  nonumber={1},
  nopages={1--33},
  year={2012},
  nopublisher={Springer}
}


@inproceedings{bartlett1992learning,
  title={Learning with a slowly changing distribution},
  author={Bartlett, Peter L},
  booktitle=COLT,
  nopages={243--252},
  year={1992}
}

@article{hanneke2020no,
  title={A no-free-lunch theorem for multitask learning},
  author={Hanneke, Steve and Kpotufe, Samory},
  journal={arXiv preprint arXiv:2006.15785},
  year={2020}
}
@inproceedings{wang2019repairing,
  title={Repairing without retraining: Avoiding disparate impact with counterfactual distributions},
  author={Wang, Hao and Ustun, Berk and Calmon, Flavio},
  booktitle=ICML,
  nopages={6618--6627},
  year={2019},
  noorganization={PMLR}
}
@inproceedings{celis2020data,
  title={Data preprocessing to mitigate bias: A maximum entropy based approach},
  author={Celis, L Elisa and Keswani, Vijay and Vishnoi, Nisheeth},
  booktitle=ICML,
  nopages={1349--1359},
  year={2020},
  noorganization={PMLR}
}
@inproceedings{donini2018empirical,
  title={Empirical risk minimization under fairness constraints},
  author={Donini, Michele and Oneto, Luca and Ben-David, Shai and Shawe-Taylor, John S and Pontil, Massimiliano},
  booktitle=NeurIPS,
  novolume={31},
  year={2018}
}
@inproceedings{calmon2017optimized,
  title={Optimized pre-processing for discrimination prevention},
  author={Calmon, Flavio and Wei, Dennis and Vinzamuri, Bhanukiran and Natesan Ramamurthy, Karthikeyan and Varshney, Kush R},
  booktitle=NeurIPS,
  novolume={30},
  year={2017}
}


@inproceedings{khetan2017learning,
  title={Learning from noisy singly-labeled data},
  author={Khetan, Ashish and Lipton, Zachary C and Anandkumar, Anima},
  booktitle=ICLR,
  year={2018}
}

@inproceedings{awasthi2017efficient,
  title={Efficient {PAC} learning from the crowd},
  author={Awasthi, Pranjal and Blum, Avrim and Haghtalab, Nika and Mansour, Yishay},
  booktitle=COLT,
  year={2017}
}




==> ablation.tex <==
\section{Ablation study: malignant versus benign manipulations}\label{sec:ablation1}
In this section, we analyze the efficacy of \method's filtering step 
and relate it to the characterization of \emph{malignant} versus 
\emph{benign} manipulations of the data.

Table~\ref{tab:filtersources} reports the fraction of 
data from manipulated sources in the training set after 
\method's \textsc{FilterSources} routine.
As one could expect, for the ID adversary, 
which by design is undetectable, the values are 
consistently at chance level. 
At the same time, our main experiments showed that this 
effect does not come with a reduction in accuracy or fairness,
since the adversary is -- also by design -- \emph{benign}: 
it does nothing, so it also does nothing bad. 

For the other adversaries, the result depends on the size and 
other characteristics of the dataset. 
For the largest \adult\ dataset, all adversaries are detected 
and filtered out perfectly. 
For the smaller \compas\ dataset, the same holds except 
for the SP adversary at $N\geq 5$ (and FL in one instance at $N=11$). 
Our main experiments show only a very slightly change in unfairness 
for this setting, though (a small increase for the fairness-regularized
methods, a small decrease for fairness-unaware training). This
confirms out initial assessment that SP is a rather benign 
manipulation. 

For the next smaller dataset, \drugs, SP is again detected the least
often, together with FL and to a lesser degree RND. For $N=11$, the
filtering also sometimes misses OL and RP.
Out of these, only FL seems to be malignant, with mainly a negative 
effect on the accuracy (fairness is sometimes even increased). The 
others have rather little influence, indicating they are rather
benign in this situation. 

For the smallest data, \german, none of the adversaries is identified 
and suppressed reliably for $N\geq 7$, and for $N\geq 9$, the filtering 
results are essentially at chance level. 
The main results showed that when learning with a fairness-unaware
base learner on this data, all adversaries except FP and SP (and ID) 
act in a malignant way and have strong impact on accuracy and/or 
fairness.
With the fairness-aware learners, however, these effects are reduced, 
with mainly FL and FB negatively influencing accuracy, and OP and 
RP having most influence on fairness. 

\begin{table}[!hbp]\centering %
\caption{Fraction of data from manipulated sources in training set after \method's \textsc{FilterSources} routine.}\label{tab:filtersources}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult\ dataset}
\begin{tabular}{c|c|c|c|c|c}
   & N=3 & N=5 & N=7 & N=9 & N=11 \\
   & {\scriptsize chance level: 0.33} & {\scriptsize chance level: 0.40} & {\scriptsize chance level: 0.43} & {\scriptsize chance level: 0.44} & {\scriptsize chance level: 0.45}\\\hline
ID & $0.30_{\pm 0.24}$ & $0.40_{\pm 0.13}$ & $0.53_{\pm 0.13}$ & $0.44_{\pm 0.17}$ & $0.43_{\pm 0.15}$\\
FP & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
FL & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
FB & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
SP & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
OP & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
OL & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
RP & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
RND & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
\end{tabular}
\end{subfigure}

\medskip\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas\ dataset}
\begin{tabular}{c|c|c|c|c|c}
   & N=3 & N=5 & N=7 & N=9 & N=11 \\
   & {\scriptsize chance level: 0.33} & {\scriptsize chance level: 0.40} & {\scriptsize chance level: 0.43} & {\scriptsize chance level: 0.44} & {\scriptsize chance level: 0.45}\\\hline
ID & $0.30_{\pm 0.24}$ & $0.47_{\pm 0.16}$ & $0.50_{\pm 0.11}$ & $0.38_{\pm 0.14}$ & $0.45_{\pm 0.08}$\\
FP & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
FL & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.08_{\pm 0.11}$\\
FB & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
SP & $0.00_{\pm 0.00}$ & $0.07_{\pm 0.13}$ & $0.35_{\pm 0.17}$ & $0.36_{\pm 0.15}$ & $0.35_{\pm 0.09}$\\
OP & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
OL & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
RP & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
RND & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.07_{\pm 0.11}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$\\
\end{tabular}
\end{subfigure}

\medskip\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs\ dataset}
\begin{tabular}{c|c|c|c|c|c}
   & N=3 & N=5 & N=7 & N=9 & N=11 \\
   & {\scriptsize chance level: 0.33} & {\scriptsize chance level: 0.40} & {\scriptsize chance level: 0.43} & {\scriptsize chance level: 0.44} & {\scriptsize chance level: 0.45}\\\hline
ID & $0.25_{\pm 0.25}$ & $0.37_{\pm 0.18}$ & $0.45_{\pm 0.19}$ & $0.50_{\pm 0.13}$ & $0.48_{\pm 0.12}$\\
FP & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.02_{\pm 0.05}$\\
FL & $0.00_{\pm 0.00}$ & $0.07_{\pm 0.20}$ & $0.25_{\pm 0.22}$ & $0.38_{\pm 0.14}$ & $0.40_{\pm 0.11}$\\
FB & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.02_{\pm 0.05}$\\
SP & $0.00_{\pm 0.00}$ & $0.03_{\pm 0.10}$ & $0.15_{\pm 0.17}$ & $0.34_{\pm 0.13}$ & $0.43_{\pm 0.11}$\\
OP & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.05_{\pm 0.11}$\\
OL & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.15_{\pm 0.17}$\\
RP & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.17_{\pm 0.22}$\\
RND & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.14_{\pm 0.09}$ & $0.12_{\pm 0.11}$\\
\end{tabular}
\end{subfigure}

\medskip\begin{subfigure}[b]{\textwidth}\centering
\caption{\german\ dataset}
\begin{tabular}{c|c|c|c|c|c}
   & N=3 & N=5 & N=7 & N=9 & N=11 \\
   & {\scriptsize chance level: 0.33} & {\scriptsize chance level: 0.40} & {\scriptsize chance level: 0.43} & {\scriptsize chance level: 0.44} & {\scriptsize chance level: 0.45}\\\hline
ID & $0.40_{\pm 0.20}$ & $0.43_{\pm 0.21}$ & $0.38_{\pm 0.12}$ & $0.50_{\pm 0.16}$ & $0.35_{\pm 0.20}$\\
FP & $0.05_{\pm 0.15}$ & $0.23_{\pm 0.15}$ & $0.30_{\pm 0.15}$ & $0.36_{\pm 0.15}$ & $0.32_{\pm 0.16}$\\
FL & $0.00_{\pm 0.00}$ & $0.20_{\pm 0.22}$ & $0.38_{\pm 0.12}$ & $0.50_{\pm 0.16}$ & $0.35_{\pm 0.20}$\\
FB & $0.00_{\pm 0.00}$ & $0.20_{\pm 0.22}$ & $0.30_{\pm 0.15}$ & $0.36_{\pm 0.15}$ & $0.32_{\pm 0.16}$\\
SP & $0.15_{\pm 0.23}$ & $0.33_{\pm 0.26}$ & $0.33_{\pm 0.16}$ & $0.44_{\pm 0.15}$ & $0.45_{\pm 0.13}$\\
OP & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.33_{\pm 0.20}$ & $0.40_{\pm 0.13}$ & $0.35_{\pm 0.12}$\\
OL & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.33_{\pm 0.16}$ & $0.48_{\pm 0.13}$ & $0.35_{\pm 0.20}$\\
RP & $0.00_{\pm 0.00}$ & $0.00_{\pm 0.00}$ & $0.45_{\pm 0.15}$ & $0.46_{\pm 0.16}$ & $0.48_{\pm 0.17}$\\
RND & $0.00_{\pm 0.00}$ & $0.10_{\pm 0.15}$ & $0.25_{\pm 0.11}$ & $0.34_{\pm 0.09}$ & $0.40_{\pm 0.20}$\\
\end{tabular}
\end{subfigure}
\end{table}


==> attic.tex <==
As our result in the following section will show, even 
these relatively simple adversaries are highly effective in 
disrupting the fairness-aware learning process. 
More complex attack strategies have also been proposed 
in the literature. \Eg, similar to~\citet{solans2020poisoning},
for real-valued input data an adversary could run a gradient-based 
optimization in order to construct data with maximally adverse effect 
on a given unfairness measure.
This would be difficult in the setting of our experiments, where 
the training data is mostly categorical.
It is also not necessary, though: for the linear classifiers that 
we consider, the effect of the data manipulations can be assessed 
explicitly, as we do above. There is no need for an attacker 
to differentiate through the model.

Either the manipulations result in measurable 
increases of the $D$-scores, and \method is able 
to identify the corresponding sources and exclude 
them from the training process. 
Or, the manipulations are such that the $D$-scores
remains small. In that case, the properties of 
disparity, discrepancy and disbalance ensure 
that the manipulations are actually harmless, 
in the sense that training on the manipulated 
data does not negatively affect accuracy or 
fairness or accuracy of the learning process



\begin{figure*}[t]
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\compas}\label{subfig:summaryresults-compas}
\includegraphics[width=.235\textwidth]{figures/compas-n5-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.235\textwidth]{figures/compas-n5-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.235\textwidth]{figures/compas-n5-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.235\textwidth]{figures/compas-n5-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\adult}\label{subfig:summaryresults-adult}
\includegraphics[width=.235\textwidth]{figures/adult-n5-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.235\textwidth]{figures/adult-n5-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.235\textwidth]{figures/adult-n5-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.235\textwidth]{figures/adult-n5-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\german}\label{subfig:summaryresults-german}
\includegraphics[width=.235\textwidth]{figures/germancredit-n5-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.235\textwidth]{figures/germancredit-n5-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.235\textwidth]{figures/germancredit-n5-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.235\textwidth]{figures/germancredit-n5-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\drugs}\label{subfig:summaryresults-drugs}
\includegraphics[width=.235\textwidth]{figures/drugs-n5-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.235\textwidth]{figures/drugs-n5-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.235\textwidth]{figures/drugs-n5-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.235\textwidth]{figures/drugs-n5-strength1000-fair-adv}
     \end{subfigure}

\caption{Results of classifier learning on data with different manipulations for baselines and \method. 
Each dataset consists of $N=5$ sources of which the adversary can manipulate $2$. The protected attribute is 
part of the feature set (larger plots and other settings can be 
found in the supplemental material).
Each subfigure contains the results for one dataset, 
split into four panels (one per baseline learner).
Each panel consists of four diagrams in a $2\times 2$ arrangement,
with top and bottom row reporting classification accuracy and 
unfairness, respectively. 
The left column ("baseline") of each panel reports the baseline 
behavior of training on the data available in the respective setting. 
The first bar ("clean", blue) shows the result of training on all 
data when no adversary is present. The remaining bars correspond 
to the situations where different adversaries have perturbed the 
data. 
The right column ("\methodname") of each panel shows the results when 
training with \method on the same data in combination with the 
respective baseline learner. 
Here, the first bar ("oracle", blue) shows the result of training 
only on the unperturbed data sources. %
The other bars show the result of training \method on data perturbed
by the respective adversaries.}
\label{fig:summaryresults}
\end{figure*}


The first panel in each figure %
shows the situation of traditional learning, 
\ie without explicitly enforcing fairness. 
One can see that even without any adversary the trained 
classifiers are not particularly fair ("baseline" column,
"clean" bar): they exhibit demographic parity violations 
of approximately 30\% (\compas and \drugs), 20\% (\adult) 
and 10\% (\german).
At the same time, the setting is highly susceptible to 
data perturbations (other bars), which depending on the
adversary affect accuracy, fairness or both.
The right column of each of these panels shows that \method 
overcomes these problems. The fairness and accuracy match the 
values when only the unperturbed part of the data is used for 
learning ("oracle" bar), even in the presence of adversaries 
(other bars).

The remaining panels illustrate the situation for the three 
different fairness-aware learning methods: regularization-based 
(panel 2), postprocessing-based~(panel 3) or adversarial~(panel 4). 
The left column of each panel shows the baseline behavior,
of training the fairness-aware learning directly on all 
available data. 
One can see that all of the fairness-aware baseline methods 
produce reasonably fair classifiers when the data is free
of manipulations ("clean" bars). 
However, in the presence of the adversaries (other bars) 
none of them is able to reliably ensure the fairness of 
the learned classifiers. 


The right column of each panel shows the result for \method 
when learning with the same given data, and the respective 
baseline as base learner. 
In every case \method reliably suppresses the effects of any 
of the adversaries, producing classifiers whose accuracy and 
fairness matches almost exactly that of a fair classifier 
trained only on the clean data sources ("oracle").

Overall, our results confirm the findings of previous works: 
\emph{fair learners do not guarantee fair classifiers, if 
the quality of the training data cannot be guaranteed}. 
At the same time, they show that protection against perturbed
data is in fact possible, as \emph{\method reliably recovers 
the accuracy and fairness of a classifier trained on only on 
unperturbed data}.




\paragraph{Adversaries}\label{subsec:adversaries}
In a real-world setting, one does not know what kind of 
data quality issues will occur. 
Therefore, we test the baselines and \method for a range 
of adversaries that reflect potentially unintentional errors 
as well as intentional manipulations. 

$\bullet$\halfquad\emph{identity (ID)}: the adversary makes 
no changes to the data. This baseline reflects the fact 
that even though the adversary has the power to 
manipulate the data it does not have to.

$\bullet$\halfquad\emph{flip protected (FP), flip label (FL), flip both (FB)}: 
the adversary flips the value of protected attribute, of the label, 
or both, in all sources it can manipulate.
FP inverts the correlations between the protected attribute and 
the other data, thereby masking a potential existing 
bias in the data. 
FL inverts the correlation of the label with the other data, 
which can hurt the classifier accuracy. FB preserves the correlation 
of protected attributes and labels, but inverts the correlation 
with all other features. This can cause the learner to rely more 
on the protected attribute for classification, thereby causing 
unfairness.
Note that FP, FL and FB could occur accidentally, \eg as problems 
during data entering, but also as active attempts to derail 
a fairness-aware learner.

$\bullet$\halfquad\emph{shuffle protected (SP)}: the adversary shuffles 
the protected attribute entry in each effected batch, \eg to hide 
the true values of the protected attributes without changing 
their proportions.
Note that the decisions of a fair learner should not be depend on the 
protected attribute anyway. Therefore, we expect the SP manipulations 
to be rather benign.

$\bullet$\halfquad\emph{overwrite protected (OP), overwrite label (OL)}: 
the adversary overwrites the protected attribute of each sample 
in the affected batch by its label, or vice versa. 
A perfect classifier for OP or OL-perturbed data is to decide 
solely based on the protected attribute, \ie it is maximally unfair.
OL can also be expected to negatively affect the classification 
accuracy, because the training labels differ from their ground-truth 
values. OP might not have that effect, but it changes the marginal 
probabilities of the protected attribute. 

$\bullet$\halfquad\emph{resample protected (RP)}: the adversary samples new 
batches of data in the following ways: all original samples of protected 
group $a=0$ with labels $y=1$ are replaced by data samples from other 
sources which also have $a=0$ but $y=0$. 
Analogously, all samples of group $a=1$ with labels $y=0$ are replaced 
by data samples from other sources with $a=1$ and $y=1$. 
Like OL and OP, RP results in a perfect correlation between protected 
attributes and labels, thereby facilitating unfairness. It does so in 
a more subtle and harder-to-detect way, though, as it achieves the 
effect using original data samples.

$\bullet$\halfquad\emph{random (RND)}: the adversary randomly picks 
one of the strategies above (except ID) for each source.

\begin{figure*}[!htbp]
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\compas}\label{subfig:summaryresults-compas}
\includegraphics[width=\textwidth]{compas-n5-fair-reg}
     \end{subfigure}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\adult}\label{subfig:summaryresults-adult}
\includegraphics[width=\textwidth]{adult-n5-fair-reg}
     \end{subfigure}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\drugs}\label{subfig:summaryresults-drugs}
\includegraphics[width=\textwidth]{drugs-n5-fair-reg}
     \end{subfigure}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\german}\label{subfig:summaryresults-german}
\includegraphics[width=\textwidth]{germancredit-n5-fair-reg}
     \end{subfigure}
\caption{Results of classifier learning on data with different manipulations 
for baselines and \method with fairness regularized base classifier. 
Each dataset consists of $N=5$ sources of which the adversary can manipulate $2$. 
The protected attribute is part of the feature set (plots for other 
settings can be found in the supplemental material).
Each subfigure consists of five panels that report results for different
training methods. The left-most is plain training without any precautions
against noisy or manipulated data. The right-most is the FLEA method we 
propose. The remaining three are possible alternative methods, 
see the main text on page~\pageref{subsec:baselines}.
Each panel contains two diagrams: the top one reports classification 
accuracy (higher is better), the bottom on unfairness (lower is better). 
The bars in the diagrams correspond to different situations of noisy 
or manipulated data.
The left-most bar ("oracle") in each diagram shows the result of 
training only on the clean data sources, \ie the ones which the 
adversary cannot modify. This is a hypothetical reference, since 
the necessary information is not available to practical algorithms.
The remaining bars correspond different adversaries perturbing the 
data, see the main text on page~\pageref{subsec:adversaries}.}
\label{fig:summaryresults}
\end{figure*}



\begin{figure*}[t]
\caption{Results of classifier learning on data with different manipulations for baselines and \method. 
Each dataset consists of $N=3$ sources of which the adversary can manipulate $1$. 
}\label{fig:summaryresults3}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\compas}\label{subfig:summaryresults-compas3}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n3-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n3-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n3-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n3-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\adult}\label{subfig:summaryresults-adult3}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n3-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n3-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n3-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n3-strength1000-fair-adv}
     \end{subfigure}
     \end{figure*}
     \begin{figure*}[t]
     \ContinuedFloat
\caption{($N=3$ continued)}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\german}\label{subfig:summaryresults-german3}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n3-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n3-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n3-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n3-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\drugs}\label{subfig:summaryresults-drugs3}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n3-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n3-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n3-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n3-strength1000-fair-adv}
     \end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{Results of classifier learning on data with different manipulations for baselines and \method. 
Each dataset consists of $N=5$ sources of which the adversary can manipulate $2$. 
}\label{fig:summaryresults5}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\compas}\label{subfig:summaryresults-compas5}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n5-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n5-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n5-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n5-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\adult}\label{subfig:summaryresults-adult5}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n5-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n5-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n5-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n5-strength1000-fair-adv}
     \end{subfigure}
     \end{figure*}
     \begin{figure*}[t]
     \ContinuedFloat\caption{($N=5$ continued)}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\german}\label{subfig:summaryresults-german5}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n5-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n5-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n5-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n5-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\drugs}\label{subfig:summaryresults-drugs5}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n5-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n5-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n5-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n5-strength1000-fair-adv}
     \end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{Results of classifier learning on data with different manipulations for baselines and \method. 
Each dataset consists of $N=7$ sources of which the adversary can manipulate $3$. 
}\label{fig:summaryresults7}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\compas}\label{subfig:summaryresults-compas7}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n7-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n7-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n7-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n7-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\adult}\label{subfig:summaryresults-adult7}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n7-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n7-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n7-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n7-strength1000-fair-adv}
     \end{subfigure}
     \end{figure*}
     \begin{figure*}[t]
     \ContinuedFloat\caption{($N=7$ continued)}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\german}\label{subfig:summaryresults-german7}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n7-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n7-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n7-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n7-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\drugs}\label{subfig:summaryresults-drugs7}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n7-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n7-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n7-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n7-strength1000-fair-adv}
     \end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{Results of classifier learning on data with different manipulations for baselines and \method. 
Each dataset consists of $N=9$ sources of which the adversary can manipulate $4$. 
}\label{fig:summaryresults9}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\compas}\label{subfig:summaryresults-compas9}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n9-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n9-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n9-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n9-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\adult}\label{subfig:summaryresults-adult9}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n9-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n9-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n9-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n9-strength1000-fair-adv}
     \end{subfigure}
     \end{figure*}
     \begin{figure*}[t]
     \ContinuedFloat\caption{($N=9$ continued)}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\german}\label{subfig:summaryresults-german9}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n9-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n9-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n9-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n9-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\drugs}\label{subfig:summaryresults-drugs9}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n9-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{figures/drugs-n9-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n9-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n9-strength1000-fair-adv}
     \end{subfigure}
\end{figure*}


\begin{figure*}[t]
\caption{Results of classifier learning on data with different manipulations for baselines and \method. 
Each dataset consists of $N=11$ sources of which the adversary can manipulate $5$. 
}\label{fig:summaryresults11}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\compas}\label{subfig:summaryresults-compas11}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n11-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n11-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n11-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{compas-n11-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\adult}\label{subfig:summaryresults-adult11}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n11-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n11-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n11-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{adult-n11-strength1000-fair-adv}
     \end{subfigure}
     \end{figure*}
     \begin{figure*}[t]
     \ContinuedFloat\caption{($N=11$ continued)}
     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\german}\label{subfig:summaryresults-german11}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n11-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n11-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n11-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{germancredit-n11-strength1000-fair-adv}
     \end{subfigure}

     \begin{subfigure}[b]{\textwidth}\centering
     \caption{\drugs}\label{subfig:summaryresults-drugs11}
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n11-strength1000-vanilla-legend}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n11-strength1000-fair-reg}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n11-strength1000-fair-pp}
\quarterquad
\includegraphics[width=.4\textwidth,height=.32\textwidth]{drugs-n11-strength1000-fair-adv}
     \end{subfigure}
\end{figure*}

\clearpage



\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n3}
\includegraphics[width=\textwidth]{suppl-compas-n3-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n3}
\includegraphics[width=\textwidth]{suppl-adult-n3-fair-reg}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n3}
\includegraphics[width=\textwidth]{suppl-drugs-n3-fair-reg}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n3}
\includegraphics[width=\textwidth]{suppl-germancredit-n3-fair-reg}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=3$ sources of which 
the adversary can manipulate $1$. Classifiers are learned
with fairness regularization. For further details, see 
Figure~\ref{fig:summaryresults}}
\label{extrafig:summaryresults_first}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n5}
\includegraphics[width=\textwidth]{suppl-compas-n5-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n5}
\includegraphics[width=\textwidth]{suppl-adult-n5-fair-reg}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n5}
\includegraphics[width=\textwidth]{suppl-drugs-n5-fair-reg}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n5}
\includegraphics[width=\textwidth]{suppl-germancredit-n5-fair-reg}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=5$ sources of which 
the adversary can manipulate $2$. Classifiers are learned
with fairness regularization. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n7}
\includegraphics[width=\textwidth]{suppl-compas-n7-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n7}
\includegraphics[width=\textwidth]{suppl-adult-n7-fair-reg}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n7}
\includegraphics[width=\textwidth]{suppl-drugs-n7-fair-reg}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n7}
\includegraphics[width=\textwidth]{suppl-germancredit-n7-fair-reg}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=7$ sources of which 
the adversary can manipulate $3$. Classifiers are learned
with fairness regularization. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n9}
\includegraphics[width=\textwidth]{suppl-compas-n9-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n9}
\includegraphics[width=\textwidth]{suppl-adult-n9-fair-reg}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n9}
\includegraphics[width=\textwidth]{suppl-drugs-n9-fair-reg}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n9}
\includegraphics[width=\textwidth]{suppl-germancredit-n9-fair-reg}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=9$ sources of which 
the adversary can manipulate $4$. Classifiers are learned
with fairness regularization. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n11}
\includegraphics[width=\textwidth]{suppl-compas-n11-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n11}
\includegraphics[width=\textwidth]{suppl-adult-n11-fair-reg}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n11}
\includegraphics[width=\textwidth]{suppl-drugs-n11-fair-reg}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n11}
\includegraphics[width=\textwidth]{suppl-germancredit-n11-fair-reg}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=11$ sources of which 
the adversary can manipulate $5$. Classifiers are learned
with fairness regularization. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}



\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n3}
\includegraphics[width=\textwidth]{suppl-compas-n3-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n3}
\includegraphics[width=\textwidth]{suppl-adult-n3-fair-pp}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n3}
\includegraphics[width=\textwidth]{suppl-drugs-n3-fair-pp}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n3}
\includegraphics[width=\textwidth]{suppl-germancredit-n3-fair-pp}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=3$ sources of which 
the adversary can manipulate $1$. Classifiers are learned
with fairness postprocessing. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n5}
\includegraphics[width=\textwidth]{suppl-compas-n5-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n5}
\includegraphics[width=\textwidth]{suppl-adult-n5-fair-pp}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n5}
\includegraphics[width=\textwidth]{suppl-drugs-n5-fair-pp}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n5}
\includegraphics[width=\textwidth]{suppl-germancredit-n5-fair-pp}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=5$ sources of which 
the adversary can manipulate $2$. Classifiers are learned
with fairness postprocessing. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n7}
\includegraphics[width=\textwidth]{suppl-compas-n7-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n7}
\includegraphics[width=\textwidth]{suppl-adult-n7-fair-pp}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n7}
\includegraphics[width=\textwidth]{suppl-drugs-n7-fair-pp}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n7}
\includegraphics[width=\textwidth]{suppl-germancredit-n7-fair-pp}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=7$ sources of which 
the adversary can manipulate $3$. Classifiers are learned
with fairness postprocessing. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n9}
\includegraphics[width=\textwidth]{suppl-compas-n9-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n9}
\includegraphics[width=\textwidth]{suppl-adult-n9-fair-pp}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n9}
\includegraphics[width=\textwidth]{suppl-drugs-n9-fair-pp}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n9}
\includegraphics[width=\textwidth]{suppl-germancredit-n9-fair-pp}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=9$ sources of which 
the adversary can manipulate $4$. Classifiers are learned
with fairness postprocessing. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n11}
\includegraphics[width=\textwidth]{suppl-compas-n11-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n11}
\includegraphics[width=\textwidth]{suppl-adult-n11-fair-pp}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n11}
\includegraphics[width=\textwidth]{suppl-drugs-n11-fair-pp}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n11}
\includegraphics[width=\textwidth]{suppl-germancredit-n11-fair-pp}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=11$ sources of which 
the adversary can manipulate $5$. Classifiers are learned
with fairness postprocessing. For further details, see 
Figure~\ref{fig:summaryresults}}
\label{extrafig:summaryresults-first}
\end{figure*}




\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n3}
\includegraphics[width=\textwidth]{suppl-compas-n3-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n3}
\includegraphics[width=\textwidth]{suppl-adult-n3-fair-adv}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n3}
\includegraphics[width=\textwidth]{suppl-drugs-n3-fair-adv}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n3}
\includegraphics[width=\textwidth]{suppl-germancredit-n3-fair-adv}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=3$ sources of which 
the adversary can manipulate $1$. Classifiers are learned
with adversarial fairness. For further details, see 
Figure~\ref{fig:summaryresults}}

\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n5}
\includegraphics[width=\textwidth]{suppl-compas-n5-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n5}
\includegraphics[width=\textwidth]{suppl-adult-n5-fair-adv}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n5}
\includegraphics[width=\textwidth]{suppl-drugs-n5-fair-adv}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n5}
\includegraphics[width=\textwidth]{suppl-germancredit-n5-fair-adv}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=5$ sources of which 
the adversary can manipulate $2$. Classifiers are learned
with adversarial fairness. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n7}
\includegraphics[width=\textwidth]{suppl-compas-n7-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n7}
\includegraphics[width=\textwidth]{suppl-adult-n7-fair-adv}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n7}
\includegraphics[width=\textwidth]{suppl-drugs-n7-fair-adv}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n7}
\includegraphics[width=\textwidth]{suppl-germancredit-n7-fair-adv}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=7$ sources of which 
the adversary can manipulate $3$. Classifiers are learned
with adversarial fairness. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n9}
\includegraphics[width=\textwidth]{suppl-compas-n9-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n9}
\includegraphics[width=\textwidth]{suppl-adult-n9-fair-adv}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n9}
\includegraphics[width=\textwidth]{suppl-drugs-n9-fair-adv}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n9}
\includegraphics[width=\textwidth]{suppl-germancredit-n9-fair-adv}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=9$ sources of which 
the adversary can manipulate $4$. Classifiers are learned
with adversarial fairness. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n11}
\includegraphics[width=\textwidth]{suppl-compas-n11-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n11}
\includegraphics[width=\textwidth]{suppl-adult-n11-fair-adv}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n11}
\includegraphics[width=\textwidth]{suppl-drugs-n11-fair-adv}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n11}
\includegraphics[width=\textwidth]{suppl-germancredit-n11-fair-adv}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=11$ sources of which 
the adversary can manipulate $5$. Classifiers are learned
with adversarial fairness. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}




\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n3}
\includegraphics[width=\textwidth]{suppl-compas-n3-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n3}
\includegraphics[width=\textwidth]{suppl-adult-n3-fair-none}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n3}
\includegraphics[width=\textwidth]{suppl-drugs-n3-fair-none}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n3}
\includegraphics[width=\textwidth]{suppl-germancredit-n3-fair-none}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=3$ sources of which 
the adversary can manipulate $1$. Classifiers are learned
without enforcing fairness. For further details, see 
Figure~\ref{fig:summaryresults}}

\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n5}
\includegraphics[width=\textwidth]{suppl-compas-n5-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n5}
\includegraphics[width=\textwidth]{suppl-adult-n5-fair-none}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n5}
\includegraphics[width=\textwidth]{suppl-drugs-n5-fair-none}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n5}
\includegraphics[width=\textwidth]{suppl-germancredit-n5-fair-none}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=5$ sources of which 
the adversary can manipulate $2$. Classifiers are learned
without enforcing fairness. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n7}
\includegraphics[width=\textwidth]{suppl-compas-n7-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n7}
\includegraphics[width=\textwidth]{suppl-adult-n7-fair-none}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n7}
\includegraphics[width=\textwidth]{suppl-drugs-n7-fair-none}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n7}
\includegraphics[width=\textwidth]{suppl-germancredit-n7-fair-none}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=7$ sources of which 
the adversary can manipulate $3$. Classifiers are learned
without enforcing fairness. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n9}
\includegraphics[width=\textwidth]{suppl-compas-n9-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n9}
\includegraphics[width=\textwidth]{suppl-adult-n9-fair-none}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n9}
\includegraphics[width=\textwidth]{suppl-drugs-n9-fair-none}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n9}
\includegraphics[width=\textwidth]{suppl-germancredit-n9-fair-none}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=9$ sources of which 
the adversary can manipulate $4$. Classifiers are learned
without enforcing fairness. For further details, see 
Figure~\ref{fig:summaryresults}}
\end{figure*}


\begin{figure*}[t]

\begin{subfigure}[b]{\textwidth}\centering
\caption{\compas}\label{subfig:summaryresults-compas-n11}
\includegraphics[width=\textwidth]{suppl-compas-n11-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{\adult}\label{subfig:summaryresults-adult-n11}
\includegraphics[width=\textwidth]{suppl-adult-n11-fair-none}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\drugs}\label{subfig:summaryresults-drugs-n11}
\includegraphics[width=\textwidth]{suppl-drugs-n11-fair-none}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}\centering
\caption{\german}\label{subfig:summaryresults-german-n11}
\includegraphics[width=\textwidth]{suppl-germancredit-n11-fair-none}
\end{subfigure}

\caption{Results of classifier learning on data with different 
manipulations. Each dataset consists of $N=11$ sources of which 
the adversary can manipulate $5$. Classifiers are learned
without enforcing fairness. For further details, see 
Figure~\ref{fig:summaryresults}}
\label{extrafig:summaryresults_last} 
\end{figure*}










\begin{table*}[t]\centering %
\caption{Fraction of manipulated data after \filter filtering.}
\label{tab:manipulatedfractionextended}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3$, $K=2$. Chance level would be $0.33$.}
\begin{tabular}{c|c|c|c|c}
adversary & compas & adult & germancredit & drugs\\\hline
FP & $0.00$ & $0.00$ & $0.05$ & $0.00$\\
FL & $0.00$ & $0.00$ & $0.00$ & $0.00$\\
FB & $0.00$ & $0.00$ & $0.00$ & $0.00$\\
SP & $0.05$ & $0.00$ & $0.25$ & $0.00$\\
OP & $0.00$ & $0.00$ & $0.00$ & $0.00$\\
OL & $0.00$ & $0.00$ & $0.00$ & $0.00$\\
RP & $0.00$ & $0.00$ & $0.00$ & $0.00$\\
\end{tabular}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5$, $K=3$. Chance level would be $0.40$.}
\label{subtab:manipulatedfractionextended5}
\begin{tabular}{c|c|c|c|c}
adversary & compas & adult & germancredit & drugs\\\hline
FP & $0.00$ & $0.00$ & $0.27$ & $0.00$\\
FL & $0.00$ & $0.00$ & $0.27$ & $0.07$\\
FB & $0.00$ & $0.00$ & $0.23$ & $0.00$\\
SP & $0.07$ & $0.00$ & $0.40$ & $0.03$\\
OP & $0.00$ & $0.00$ & $0.00$ & $0.00$\\
OL & $0.00$ & $0.00$ & $0.00$ & $0.00$\\
RP & $0.00$ & $0.00$ & $0.00$ & $0.00$\\
\end{tabular}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7$, $K=4$. Chance level would be $0.43$.}
\begin{tabular}{c|c|c|c|c}
adversary & compas & adult & germancredit & drugs\\\hline
FP & $0.00$ & $0.00$ & $0.30$ & $0.00$\\
FL & $0.00$ & $0.00$ & $0.35$ & $0.25$\\
FB & $0.00$ & $0.00$ & $0.30$ & $0.00$\\
SP & $0.25$ & $0.00$ & $0.42$ & $0.10$\\
OP & $0.00$ & $0.00$ & $0.38$ & $0.00$\\
OL & $0.00$ & $0.00$ & $0.30$ & $0.00$\\
RP & $0.00$ & $0.00$ & $0.42$ & $0.00$\\
\end{tabular}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9$, $K=5$. Chance level would be $0.44$.}
\begin{tabular}{c|c|c|c|c}
adversary & compas & adult & germancredit & drugs\\\hline
FP & $0.00$ & $0.00$ & $0.32$ & $0.00$\\
FL & $0.00$ & $0.00$ & $0.42$ & $0.36$\\
FB & $0.00$ & $0.00$ & $0.32$ & $0.00$\\
SP & $0.28$ & $0.00$ & $0.42$ & $0.36$\\
OP & $0.00$ & $0.00$ & $0.42$ & $0.00$\\
OL & $0.00$ & $0.00$ & $0.42$ & $0.00$\\
RP & $0.00$ & $0.00$ & $0.46$ & $0.00$\\
\end{tabular}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11$, $K=6$. Chance level would be $0.45$.}
\begin{tabular}{c|c|c|c|c}
adversary & compas & adult & germancredit & drugs\\\hline
FP & $0.00$ & $0.00$ & $0.32$ & $0.02$\\
FL & $0.08$ & $0.00$ & $0.38$ & $0.40$\\
FB & $0.00$ & $0.00$ & $0.32$ & $0.02$\\
SP & $0.28$ & $0.00$ & $0.40$ & $0.38$\\
OP & $0.00$ & $0.00$ & $0.40$ & $0.05$\\
OL & $0.00$ & $0.00$ & $0.38$ & $0.13$\\
RP & $0.00$ & $0.00$ & $0.55$ & $0.13$\\
\end{tabular}
\end{subfigure}
\end{table*}

\subsection{Ablation study: role of disparity, discrepancy and disbalance}
\method is based on the combination of three dissimilarity measures:
discrepancy, disparity and disbalance. Here we analyze the role 
of each component, showing that their combination leads to better 
decisions than any individual component. 

Table~\ref{tab:manipulatedfractionablation} shows the fraction 
of manipulated data sources that pass the \filter stage, either 
for \method's $D$-score or for a procedure that uses the same 
steps but relies only each of the individual measures. 

One can see that the discrepancy is often successful in identifying 
manipulations, but it tends to fail for adversaries that concentrate 
on manipulating the protected attribute (FP and sometimes SP). 
By its definitions, the discrepancy is not able to identify 
manipulations of the labels (FL, OL). It is also most affected 
by small sample size of the three measures. The disbalance, also 
by definition, can only identity adversaries that manipulate the 
marginal probabilities of the protected attribute. 
Their combination generally works at least as good as each individual 
measure, except for a few cases on the small datasets \german and \drugs. 
There, we observed the disparity to take generally rather large 
values and dominate the combination. 

\begin{table*}[h]\centering \footnotesize
\caption{Fraction of manipulated data after filtering with only disparity, 
only discrepancy, and disbalance or their combination (\ie \method).}
\label{tab:manipulatedfractionablation}
\begin{subfigure}[b]{.6\textwidth}\centering
\caption{\texttt{compas} ($N=5$, $K=3$)}
\begin{tabular}{c|c|c|c|c} %
opponent & \method & $\disc$-only & $\disp$-only  & $\disb$-only\\\hline
FP & 0.00 & 0.37 & 0.00 & 0.00\\
FL & 0.00 & 0.00 & 0.43 & 0.57\\
FB & 0.00 & 0.00 & 0.00 & 0.00\\
SP & 0.07 & 0.33 & 0.07 & 0.57\\
OP & 0.00 & 0.00 & 0.00 & 0.00\\
OL & 0.00 & 0.00 & 0.43 & 0.57\\
RP & 0.00 & 0.00 & 0.00 & 0.57\\
\end{tabular}
\end{subfigure}
\begin{subfigure}[b]{.6\textwidth}\centering
\caption{\texttt{adult} ($N=5$, $K=3$)}
\begin{tabular}{c|c|c|c|c} %
opponent & \method & $\disc$-only & $\disp$-only  & $\disb$-only\\\hline
FP & 0.00 & 0.40 & 0.00 & 0.00\\
FL & 0.00 & 0.00 & 0.37 & 0.47\\
FB & 0.00 & 0.00 & 0.00 & 0.00\\
SP & 0.00 & 0.00 & 0.00 & 0.47\\
OP & 0.00 & 0.00 & 0.00 & 0.00\\
OL & 0.00 & 0.00 & 0.37 & 0.47\\
RP & 0.00 & 0.00 & 0.00 & 0.47\\
\end{tabular}
\end{subfigure}
\begin{subfigure}[b]{.6\textwidth}\centering
\caption{\texttt{germancredit} ($N=5$, $K=3$)}
\begin{tabular}{c|c|c|c|c} %
opponent & \method & $\disc$-only & $\disp$-only  & $\disb$-only\\\hline
FP & 0.27 & 0.13 & 0.27 & 0.00\\
FL & 0.27 & 0.00 & 0.43 & 0.27\\
FB & 0.23 & 0.00 & 0.27 & 0.00\\
SP & 0.40 & 0.33 & 0.40 & 0.27\\
OP & 0.00 & 0.00 & 0.27 & 0.00\\
OL & 0.00 & 0.00 & 0.43 & 0.27\\
RP & 0.00 & 0.00 & 0.37 & 0.27\\
\end{tabular}
\end{subfigure}
\begin{subfigure}[b]{.6\textwidth}\centering
\caption{\texttt{drugs} ($N=5$, $K=3$)}
\begin{tabular}{c|c|c|c|c} %
opponent & \method & $\disc$-only & $\disp$-only  & $\disb$-only\\\hline
FP & 0.00 & 0.13 & 0.00 & 0.30\\
FL & 0.07 & 0.00 & 0.40 & 0.33\\
FB & 0.00 & 0.00 & 0.00 & 0.30\\
SP & 0.03 & 0.33 & 0.03 & 0.33\\
OP & 0.00 & 0.00 & 0.00 & 0.30\\
OL & 0.00 & 0.00 & 0.40 & 0.33\\
RP & 0.00 & 0.00 & 0.10 & 0.33\\
\end{tabular}
\end{subfigure}
\end{table*}


\subsection{Alternative approach: robust ensembles}
\textcolor{red}{Present together with other baselines.}

One can imagine other ways how to deal with potentially 
unreliably sources rather than filtering. For example, 
train individual classifiers on each available dataset 
and predict by evaluating all classifiers and returning 
the median predicted score. 
This \emph{robust ensemble} learner can be expected to 
show robustness as well, since if all classifiers that were 
trained on clean sources agree on their decision, the median 
would take the same value. 
A drawback is that this construction cannot make use of 
potentially available information what fraction of sources 
are clean. 
We benchmarked this method in the same setting as \method. 
Figure~\ref{fig:summarensemble5} shows the result for $N=5$.
Indeed one can see that the effect of some adversaries
is mitigated or removed. However, in some cases, the
unfairness is even increased. Overall the method is 
clearly less robust and effective than \method.





\begin{table*}[t]\centering\footnotesize
\begin{tabular}{l|ll|ll|ll|ll}
& \multicolumn{2}{c}{\adult} & \multicolumn{2}{c}{\compas} & \multicolumn{2}{c}{\drugs} & \multicolumn{2}{c}{\german}
\\
\textbf{method} & accuracy & fairness & accuracy & fairness & accuracy & fairness & accuracy & fairness 
\\\hline
\color{red}vanilla	        & $66.2_{\pm 1.1}$ & $77.6_{\pm 1.2}$ & $63.5_{\pm 2.1}$ & $78.9_{\pm 2.3}$  & $60.1_{\pm 2.5}$ & $72.3_{\pm 3.1}$ & $58.1_{\pm 4.0}$ & $81.9_{\pm 5.0}$
\\
ensemble	      & $69.9_{\pm 0.4}$& $90.9_{\pm 1.6}$& $65.0_{\pm 1.1}$& $88.4_{\pm 2.9}$& $61.0_{\pm 2.1}$& $75.7_{\pm 5.2}$& $62.1_{\pm 2.9}$& $71.2_{\pm 7.0}$
\\
DRO	 []         & $52.8_{\pm 0.3}$ & $15.4_{\pm 1.3}$ & $54.5_{\pm 1.2}$ & $70.9_{\pm 5.7}$ & $55.1_{\pm 2.5}$ & $53.9_{\pm 23.3}$ & $65.0_{\pm 4.9}$ & $78.4_{\pm 13.1}$
\\
Konstantinov []	& $69.3_{\pm 0.4}$ & $77.6_{\pm 1.2}$ & $63.5_{\pm 2.1}$ & $78.9_{\pm 2.3}$ & $60.1_{\pm 2.5}$ & $72.3_{\pm 3.1}$ & $58.1_{\pm 4.0}$ & $81.9_{\pm 5.0}$
\\
\color{blue}FLEA (proposed) & $70.3_{\pm 0.4}$ & $98.0_{\pm 1.1}$ & $65.8_{\pm 1.0}$ & $95.6_{\pm 1.9}$ & $60.8_{\pm 8.3}$ & $91.5_{\pm 2.9}$ & $60.5_{\pm 8.7}$ & $89.7_{\pm 4.9}$
\\
\color{green}oracle	        & $70.3_{\pm 0.4}$ & $98.2_{\pm 1.0}$ & $66.2_{\pm 1.1}$ & $96.2_{\pm 1.3}$ & $64.4_{\pm 1.5}$ & $93.6_{\pm 3.3}$ & $67.3_{\pm 3.0}$ & $94.4_{\pm 4.0}$
\end{tabular}
\caption{like this?}
\label{tab:results-homogeneous}
\end{table*}

\begin{table}[t]\centering\small
\begin{tabular}{l|cccc}
\textbf{method} & \multicolumn{1}{c}{\adult} & \multicolumn{1}{c}{\compas} & \multicolumn{1}{c}{\drugs} & \multicolumn{1}{c}{\parbox{.15\columnwidth}{\texttt{german}\\[-.4\baselineskip]\texttt{credit}\smallskip}}
\\\hline
\color{red}vanilla  & $66.2_{\pm 1.1}$ & $63.5_{\pm 2.1}$ & $60.1_{\pm 2.5}$ & $58.1_{\pm 4.0}$  \\
                    & $77.6_{\pm 1.2}$ & $78.9_{\pm 2.3}$ & $72.3_{\pm 3.1}$ & $81.9_{\pm 5.0}$\\\hline
ensemble	          & $69.9_{\pm 0.4}$ & $65.0_{\pm 1.1}$ & $61.0_{\pm 2.1}$ & $62.1_{\pm 2.9}$ \\
                    & $90.9_{\pm 1.6}$ & $88.4_{\pm 2.9}$ & $75.7_{\pm 5.2}$ & $71.2_{\pm 7.0}$ \\\hline
DRO	 []             & $52.8_{\pm 0.3}$ & $54.5_{\pm 1.2}$ & $55.1_{\pm 2.5}$ & $65.0_{\pm 4.9}$ \\
                    & $15.4_{\pm 1.3}$ & $70.9_{\pm 5.7}$ & $53.9_{\pm 23.3}$ & $78.4_{\pm 13.1}$\\\hline
Konst. []	    & $69.3_{\pm 0.4}$ & $63.5_{\pm 2.1}$ & $60.1_{\pm 2.5}$ & $58.1_{\pm 4.0}$  \\
                    & $77.6_{\pm 1.2}$ & $78.9_{\pm 2.3}$ & $72.3_{\pm 3.1}$ & $81.9_{\pm 5.0}$  \\\hline
\color{blue}FLEA 
                    & $70.3_{\pm 0.4}$ & $65.8_{\pm 1.0}$ & $60.8_{\pm 8.3}$ & $60.5_{\pm 8.7}$ \\
                    & $98.0_{\pm 1.1}$ & $95.6_{\pm 1.9}$ & $91.5_{\pm 2.9}$ & $89.7_{\pm 4.9}$ \\\hline
\color{green}oracle	& $70.3_{\pm 0.4}$ & $66.2_{\pm 1.1}$ & $64.4_{\pm 1.5}$ & $67.3_{\pm 3.0}$ \\
                    & $98.2_{\pm 1.0}$ & $96.2_{\pm 1.3}$ & $93.6_{\pm 3.3}$ & $94.4_{\pm 4.0}$ \\\hline
\end{tabular}
\caption{or like this?}
\label{tab:results-homogeneous-singlecol}
\end{table}
\color{blue}FLEA (max) & $70.3_{\pm 0.4}$ & $98.0_{\pm 1.1}$ & $65.8_{\pm 1.0}$ & $95.6_{\pm 1.9}$ & $60.8_{\pm 8.3}$ & $91.5_{\pm 2.9}$ & $60.5_{\pm 8.7}$ & $89.7_{\pm 4.9}$
\\
\color{blue}FLEA (max)      & $75.4_{\pm 0.2}$ & $99.5_{\pm 0.3}$ & $75.4_{\pm 0.2}$ & $99.4_{\pm 0.3}$ & $75.3_{\pm 0.2}$ & $99.5_{\pm 0.3}$ & $75.3_{\pm 0.2}$ & $99.0_{\pm 0.6}$ & $63.5_{\pm 18.1}$ & $82.9_{\pm 15.8}$
\\


==> relatedwork.tex <==
\section{Related work}

To our knowledge, our work is the first one to propose an 
experimentally validated practical algorithm for learning from 
multisource data with adversarial perturbations, and also the 
first to provide theoretical guarantees for the possibility of 
learning in this scenario. 
The theoretical foundations is most closely related to 
\citet{konstantinov2020sample}, which proposes the Empirical 
Discrepancy, originally described in as the criterion for detecting 
adversarially perturbed sources in the case where data is learned from 
multiple sources each of which samples \iid from the same 
distribution. Our work improves on this work in two important ways: by 
extending this approach to the case of fairness-aware learning, and by 
proposing a practical algorithm for learning in this scenario and 
demonstrating its efficacy. Below, we summarize other works that study 
fairness-aware learning, and works that study data perturbations with 
no emphasis on fairness.

 \paragraph{Fairness-aware learning} The larger field of fairness-aware 
 learning, and specifically fairness-aware learning in the presence of 
 corrupted data, has been rapidly gaining popularity. 
 
 Several recent works \citep{woodworth2017learning,ushabat2020sample} have 
 demonstrated uniform convergence properties for specific fairness 
 metrics, while \citet{agarwal2018reductions} takes a broader view by 
 breaking multiple fairness metrics down into a series of constrained 
 optimization problems.

\done{Other works \citep{pmlr-v97-mahloujifar19a,qiao2018outliers} 
have examined poisoning attacks and their ability to severely impede 
learning in the absence of corrective action.}
\citet{mehrabi2020exacerbating} likewise demonstrates that fairness 
attacks can severely distort fairness in the final models. 
\citet{kallus2019assessing} examines biased data and demonstrates that 
even imposing fairness constraints does not fully solve the problem, as 
second-order unfairness issues may remain.

Recently, methods have been proposed for overcoming the loss of 
fairness when learning from unreliable training data.
However, so far, only a few special cases were addressed: 
in~\citet{celis2021fair, mehrotra2021setselection, roh20FRtrain, wang2020robustfairnessnoise} 
the goal is to cover fairness when the protected attribute 
itself is corrupted or noisy. 
This, however, typically comes at a loss of accuracy, and 
it requires additional information, such as a known noise 
model or a noise clean reference dataset.

\citet{celis2021adversarial} tackles the scenario where the adversary
may make arbitrary perturbations to the protected features of a proportion of the data; 
however, as this work is in the single-source scenario, the algorithm 
proposed by the authors is not optimal for the multisource scenario 
and, therefore, has weaker guarantees.

In~\citet{blum2020recovering,biswas2021ensuring} propose methods
to tackle the case when the label distribution of the training 
set differs from the true one.

However, none of the existing methods, tackle the case of 
arbitrary changes in the training data, as we do. Furthermore,
recent theoretical results~\citep{konstantinov2022theotherone}
indicate that a general solution to the problem of robust
learning with fairness is impossible in the case of a single
data batch.

\paragraph{Detecting and neutralizing in the presence of data 
perturbations} The same empirical discrepancy criterion that we use was 
first proposed by \citet{mohri2012new}, where it was used for measuring 
distribution drift. The idea of using a discrepancy-like metric is also 
used in \citet{cortes_adaptation} and \citet{zhang2012generalizationNIPS}, who use a dataset discrepancy 
metric to eliminate or downweight likely corrupted data sources or 
processing nodes when combining data. Of these, the work of 
\citet{cortes_adaptation} is perhaps the most similar, in using a 
label-agnostic version of empirical discrepancy tailored to the 
hypothesis class to assign a trust score to various samples for 
estimating the outlying distribution. However, this work focuses on 
domain adaptation, does not use labels, and is not applicable directly 
to fairness-constrained optimization problems.  Finally, the works of 
\citet{qiao2018learning}, \citet{chen2019efficiently}, 
\citet{jain2020_optimalrobustlearning} also follow a similar approach 
of estimating a distribution from partially-corrupted multisource data 
using a statistically founded discrepancy-like metric to select trusted 
data sources; however, these works focus specifically on learning 
discrete distributions and are not directly applicable to the problem 
that we consider. 



==> results-figures.tex <==
\begin{figure*}[t]
\caption{\adult\ dataset, regularization-based fairness}
\label{extrafig:summaryresults_first}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{adult-n3-N1-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{adult-n5-N2-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{adult-n7-N3-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{adult-n9-N4-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{adult-n11-N5-fair-reg}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\adult\ dataset, preprocessing-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-adult-n3-N1-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-adult-n5-N2-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-adult-n7-N3-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-adult-n9-N4-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-adult-n11-N5-fair-resample}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\adult\ dataset, postprocessing-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-adult-n3-N1-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-adult-n5-N2-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-adult-n7-N3-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-adult-n9-N4-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-adult-n11-N5-fair-pp}
\end{subfigure}
\end{figure*}


\begin{figure*}[t]
\caption{\adult\ dataset, adversarial fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-adult-n3-N1-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-adult-n5-N2-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-adult-n7-N3-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-adult-n9-N4-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-adult-n11-N5-fair-adv}
\end{subfigure}
\end{figure*}


\begin{figure*}[t]
\caption{\adult\ dataset, fairness-unaware}\label{extrafig:summaryresults_last} 
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-adult-n3-N1-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-adult-n5-N2-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-adult-n7-N3-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-adult-n9-N4-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-adult-n11-N5-fair-none}
\end{subfigure}
\end{figure*}



\begin{figure*}[t]
\caption{\compas\ dataset, regularization-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{compas-n3-N1-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{compas-n5-N2-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{compas-n7-N3-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{compas-n9-N4-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{compas-n11-N5-fair-reg}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\compas\ dataset, preprocessing-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-compas-n3-N1-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-compas-n5-N2-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-compas-n7-N3-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-compas-n9-N4-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-compas-n11-N5-fair-resample}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\compas\ dataset, postprocessing-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-compas-n3-N1-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-compas-n5-N2-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-compas-n7-N3-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-compas-n9-N4-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-compas-n11-N5-fair-pp}
\end{subfigure}
\end{figure*}


\begin{figure*}[t]
\caption{\compas\ dataset, adversarial fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-compas-n3-N1-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-compas-n5-N2-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-compas-n7-N3-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-compas-n9-N4-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-compas-n11-N5-fair-adv}
\end{subfigure}
\end{figure*}


\begin{figure*}[t]
\caption{\compas\ dataset, fairness-unaware}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-compas-n3-N1-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-compas-n5-N2-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-compas-n7-N3-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-compas-n9-N4-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-compas-n11-N5-fair-none}
\end{subfigure}
\end{figure*}



\begin{figure*}[t]
\caption{\drugs\ dataset, regularization-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{drugs-n3-N1-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{drugs-n5-N2-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{drugs-n7-N3-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{drugs-n9-N4-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{drugs-n11-N5-fair-reg}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\drugs\ dataset, preprocessing-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-drugs-n3-N1-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-drugs-n5-N2-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-drugs-n7-N3-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-drugs-n9-N4-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-drugs-n11-N5-fair-resample}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\drugs\ dataset, postprocessing-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-drugs-n3-N1-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-drugs-n5-N2-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-drugs-n7-N3-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-drugs-n9-N4-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-drugs-n11-N5-fair-pp}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\drugs\ dataset, adversarial fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-drugs-n3-N1-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-drugs-n5-N2-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-drugs-n7-N3-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-drugs-n9-N4-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-drugs-n11-N5-fair-adv}
\end{subfigure}
\end{figure*}


\begin{figure*}[t]
\caption{\drugs\ dataset, fairness-unaware}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-drugs-n3-N1-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-drugs-n5-N2-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-drugs-n7-N3-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-drugs-n9-N4-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-drugs-n11-N5-fair-none}
\end{subfigure}
\end{figure*}



\begin{figure*}[t]
\caption{\german\ dataset, regularization-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{germancredit-n3-N1-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{germancredit-n5-N2-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{germancredit-n7-N3-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{germancredit-n9-N4-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{germancredit-n11-N5-fair-reg}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\german\ dataset, preprocessing-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-germancredit-n3-N1-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-germancredit-n5-N2-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-germancredit-n7-N3-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-germancredit-n9-N4-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-germancredit-n11-N5-fair-resample}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\german\ dataset, postprocessing-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-germancredit-n3-N1-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-germancredit-n5-N2-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-germancredit-n7-N3-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-germancredit-n9-N4-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-germancredit-n11-N5-fair-pp}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\german\ dataset, adversarial fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-germancredit-n3-N1-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-germancredit-n5-N2-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-germancredit-n7-N3-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-germancredit-n9-N4-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-germancredit-n11-N5-fair-adv}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\german\ dataset, fairness-unaware}
\label{extrafig:summaryresults_last} 
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=3, N-K=1$}\includegraphics[width=\textwidth]{suppl-germancredit-n3-N1-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=5, N-K=2$}\includegraphics[width=\textwidth]{suppl-germancredit-n5-N2-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=7, N-K=3$}\includegraphics[width=\textwidth]{suppl-germancredit-n7-N3-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=9, N-K=4$}\includegraphics[width=\textwidth]{suppl-germancredit-n9-N4-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=11, N-K=5$}\includegraphics[width=\textwidth]{suppl-germancredit-n11-N5-fair-none}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\folktables\ dataset, regularization-based fairness}
\label{extrafig:summaryresults_folktables_first} 
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=5$}\includegraphics[width=\textwidth]{folktables-n51-N5-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=10$}\includegraphics[width=\textwidth]{folktables-n51-N10-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=15$}\includegraphics[width=\textwidth]{folktables-n51-N15-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=20$}\includegraphics[width=\textwidth]{folktables-n51-N20-fair-reg}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=25$}\includegraphics[width=\textwidth]{folktables-n51-N25-fair-reg}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\folktables\ dataset, preprocessing-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=5$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N5-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=10$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N10-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=15$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N15-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=20$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N20-fair-resample}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=25$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N25-fair-resample}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\folktables\ dataset, postprocessing-based fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=5$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N5-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=10$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N10-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=15$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N15-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=20$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N20-fair-pp}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=25$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N25-fair-pp}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\folktables\ dataset, adversarial fairness}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=5$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N5-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=10$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N10-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=15$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N15-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=20$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N20-fair-adv}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=25$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N25-fair-adv}
\end{subfigure}
\end{figure*}

\begin{figure*}[t]
\caption{\folktables\ dataset, fairness-unaware}
\label{extrafig:summaryresults_folktables_last} 
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=5$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N5-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=10$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N10-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=15$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N15-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=20$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N20-fair-none}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}\centering
\caption{$N=51, N-K=25$}\includegraphics[width=\textwidth]{suppl-folktables-n51-N25-fair-none}
\end{subfigure}
\end{figure*}


==> table-results-ablation-fair_adv.tex <==
# fairalgo= none
adult & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
compas & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
drugs & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
germancredit & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=5$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=10$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=15$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=20$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=25$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline


==> table-results-ablation-fair_none.tex <==
# fairalgo= none
adult & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
compas & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
drugs & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
germancredit & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=5$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=10$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=15$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=20$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=25$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline


==> table-results-ablation-fair_pp.tex <==
# fairalgo= none
adult & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
compas & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
drugs & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
germancredit & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=5$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=10$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=15$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=20$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=25$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline


==> table-results-ablation-fair_resample.tex <==
# fairalgo= none
adult & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
compas & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
drugs & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
germancredit & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=5$, $N-K=2$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=5$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=10$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=15$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=20$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline
# fairalgo= none
folktables & A:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\
$N=51$, $N-K=25$ & F:& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$& $nan_{\pm nan}$\\\hline

